Heuristic Time Complexity of NISQ Shortest-Vector-Problem Solvers

Shortest Vector Problem is believed to be hard both for classical and quantum computers. Two of the three NIST post-quantum cryptosystems standardised by NIST rely on its hardness. Research on theoretical and practical performance of quantum algorithms to solve SVP is crucial to establish confidence in them. Exploring the capabilities that Variational Quantum Algorithms (VQA) that can run on NISQ devices have in solving SVP has been an active research area. The qubit-requirement for doing so has been analysed and it was demonstrated that it is plausible to encode SVP on the ground state of a Hamiltonian efficiently. Due to the heuristic nature of VQAs no analysis of the time complexity of those approaches for scales beyond the non-interesting classically simulatable sizes has been performed. Motivated by Boulebnane and Montanaro work on the k-SAT problem, we propose to use angle pretraining of the QAOA for SVP and we demonstrate that it performs well on much larger instances than those used in training. Avoiding the limitations that arise due to the use of optimiser, we are able to extrapolate the observed performance and observe the probability of success scaling as $2^{-0.695n}$ with n being dimensionality of the search space for a depth $p=3$ pre-trained QAOA. We observe time heuristic complexity $O(2^{0.695n})$, a bit worse than the fault-tolerant Grover approach of $O(2^{0.5n})$. However, both the number of qubits, and the depth of each quantum computation, are considerably better-Grover requires exponential depth, while each run of constant p fixed-angles QAOA requires polynomial depth. We also propose a novel method to avoid the zero vector solution to SVP without introducing more logical qubits. This improves upon the previous works as it results in more space efficient encoding of SVP on NISQ architectures without ignoring the zero vector problem.

==> chapters/app_generatingGramians.tex <==
\begin{prop}\label{prop:basis_qary}
	Let $m\geq n$. Given $A\in\mathbb{Z}_q^{m\times n}=\begin{pmatrix}
		A_1\in\mathbb{Z}_q^{n\times n} \\ A_2\in\mathbb{Z}_q^{(m-n)\times n}
	\end{pmatrix}$ such that $A_1$ is invertible in $\mathbb{Z}_q$,
	\begin{equation*}
		B_A=\begin{pmatrix} I_n & A_1^{-1}A_2 \\ 0 & qI_{m-n} \end{pmatrix}\in\mathbb{Z}^{m\times m}
	\end{equation*}is a lattice basis for $\Lambda_q(A)$, i.e. $\lattice(B_A)=\Lambda_q(A)$.
\end{prop}
\begin{proof}
	Observe that \begin{align*}
		x=\begin{pmatrix}
			x_1\in\mathbb{Z}^{1\times n} & x_2\in\mathbb{Z}^{1\times (m-n)}
		\end{pmatrix}\in\lattice(B_A)\iff &\exists s: x \equiv sA\mod q\\
		\iff &\exists s:x_1\equiv sA_1\mod q\text{\ \ and\ \ }x_2\equiv sA_2\mod q\\
		\iff &\exists s:x_1A_1^{-1}\equiv s\mod q\text{\ \ and\ \ }x_2\equiv (x_1A_1^{-1})A_2\mod q\\
		\iff &\exists s:x_1A_1^{-1}\equiv s\mod q\text{\ \ and\ \ }x_2\equiv x_1A_1^{-1}A_2+qz\\
		&\text{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  for any \ }z\in\mathbb{Z}^{1\times (m-n)}
	\end{align*}
	Let $x=\begin{pmatrix}
		x_1\in\mathbb{Z}^{1\times n} & x_2\in\mathbb{Z}^{1\times (m-n)}
	\end{pmatrix}\in\mathbb{Z}^{1\times m}$, we proceed to show $xB_A\in\lattice(B_A)$:
	\begin{align*}
		xB_A=\begin{pmatrix}x_1&x_2\end{pmatrix}\begin{pmatrix} I_n &  A_1^{-1}A_2  \\ 0 & qI_{m-n} \end{pmatrix}=\begin{pmatrix}
			x_1&x_1A_1^{-1}A_2+qx_2
		\end{pmatrix}\in\lattice(B_A)
	\end{align*}
\end{proof}

\begin{prop}
	Let $B_A=\begin{pmatrix} I_n & A_1^{-1}A_2 \\ 0 & qI_{m-n} \end{pmatrix}$ be a basis of the lattice $\Lambda_q(A)$ as in Proposition \ref{prop:basis_qary}. Then
	\begin{align}
		B_A^\perp=\begin{pmatrix}
			qI_n &0 \\
			-A_2^T(A_1^{-1})^T & I_{m-n}
		\end{pmatrix}
	\end{align}
	is a basis of $\Lambda_q^\perp(A)$.
\end{prop}
\begin{proof}
	Observe that $B_A^T(q^{-1}B_A^\perp)=I_{m\times m}\implies q^{-1}B_A^\perp=B_A^{-T}\implies q^{-1}B_A^\perp=:B_A^*$. Because $B$ is full-rank by being lower-triangular with all diagonal entries being non-zero, the result follows from Theorem \ref{thm:dualBasis}. Note that in application of the Theorem we ignored the constant factor $q^{-1}$ as a multiplication of lattice basis by a constant does not change any underlying structure of the lattice and by ignoring it, we end up with a clean analytical form. Same approach has been followed in literature \textcolor{red}{find citation}.
\end{proof}

%\begin{prop}\label{prop:a1m1invertible}
%	Let $A=\begin{pmatrix}
	%		A_1\in\mathbb{Z}_q^{n\times n}\vert A_2\in\mathbb{Z}_q^{n\times (m-n)}
	%	\end{pmatrix}$ with $P(A=a)\sim\mathcal{U}(\mathbb{Z}^{n\times m})$ be uniformly generated over all matrices $a$ in $\mathbb{Z}^{n\times m}$. If $A_1$ is invertible over $\mathbb{Z}_q$, then $P(A_1^{-1}=b)\sim\mathcal{U}(\mathbb{Z}^{n\times n})$ is also uniformly distributed over all matrices $b$ in $\mathbb{Z}^{n\times n}$.
%\end{prop}
%\begin{proof}
%	The result follows from inverse being a bijection $GL_n(\mathbb{Z}_q)\rightarrow GL_n(\mathbb{Z}_q)$.
%\end{proof}
\begin{prop}\label{prop:uniformmultiplication}
	Let $A=\begin{pmatrix}
		A_1\in\mathbb{Z}_q^{n\times n} \\ A_2\in\mathbb{Z}_q^{(m-n)\times n}
	\end{pmatrix}$ with $A_1$ being invertible over $\mathbb{Z}^{n\times n}$ and $P(A_2=x)=p$ be uniformly generated over all matrices $x\in\mathbb{Z}_q^{n\times (m-n)}$ and let $H=A_1^{-1}A_2$. Then $P(H=h)=p$ is uniformly distributed over all matrices $h\in\mathbb{Z}_q^{n\times (m-n)}$.
\end{prop}
\begin{proof}
	\begin{align*}
		P(H=h)&=\sum_{a}P(H=h|A_1=a)P(A_1=a)\\&
		\text{because $a\in GL_n(\mathbb{Z}_q)$: $h=xa\iff x=ha^{-1}$}\\
		&=\sum_{a}P(A_2=ha^{-1}|A_1=a)P(A_1=a)\\&
		\text{by independence of $A_1$ and $A_2$}\\
		&=\sum_{a}P(A_2=ha^{-1})P(A_1=a)\\
		&\text{because $ha^{-1}\in\mathbb{Z}_1^{n\times (m-n)}$}\\
		&=\sum_{a}pP(A_1=a)\\
		&=p
	\end{align*}
	%https://math.stackexchange.com/questions/4457436/multiplication-of-two-random-matrices-over-a-finite-field
\end{proof}

\begin{prop}\label{prop:gramqary}Let $K\in\mathbb{Z}_q^{n\times (m-n)}$ be uniformly distributed random matrix. Then
	$G:=\begin{pmatrix}
		q^2I_{n\times n} & K\\
		K^T & I_{m-n}+K^TK
	\end{pmatrix}$ is a Gram matrix of an instance of a q-ary lattice basis.
\end{prop}
\begin{proof}
	A Gram matrix of the basis of $\lattice(B_A^\perp)$ can be expressed as $G:=B_A^\perp(B_A^\perp)^T=\begin{pmatrix}
		q^2I_{n\times n} & -A_1^{-1}A_2\\
		-A_2^TA_1^{-T} & I_{m-n}+A_2^TA_1^{-T}A_1^{-1}A_2
	\end{pmatrix}$. By Proposition \ref{prop:uniformmultiplication}, $P(K=k)=p$, with $K:= -A_1^{-1}A_2$, is uniformly distributed over all matrices $k\in\mathbb{Z}_q^{n\times (m-n)}$.
\end{proof}

==> chapters/figures/app_calcBestFit.tex <==
Pre-training of Fixed-angle \qaoa and Fixed-angle CM-QAOA requires a few non obvious choices for the cost function being used and the procedure to estimate the algorithmic performance given some particular trial set of angles. In \Cref{sec:appCalcBestFit_costFn} we introduce the cost function that we found to perform well during our pre-training method. It involves estimation of an exponent of a best-fit, which is then discussed in \Cref{sec:appCalcBestFit_expFit}.
\subsection{The cost function used in parameter pretraining}\label{sec:appCalcBestFit_costFn}
The parameter pretraining method of Fixed-angle QAOA and Fixed-angle CM-QAOA finds the optimal angles \(\bm{\beta}^\text{opt},\bm{\gamma}^\text{opt}\) that result in a \textit{good} performance over the training dataset \(\bm{\mathcal{L}}^{m_{\text{start}}}_{\text{train}},\bm{\mathcal{L}}^{m_{\text{start}+1}}_{\text{train}}\dots,\bm{\mathcal{L}}^{m_{\text{end}}}_{\text{train}}\). The \textit{good} performance can be understood in terms of different metrics which are encoded in the cost function \(c_\text{train}(\bm{P}_{\text{train}}(\bm{\beta},\bm{\gamma}))\) used in the optimisation. We have found two implementations of the cost function,  \(c^1_\text{train}(\bm{P}_{\text{train}}(\bm{\beta},\bm{\gamma}))\) and \(c^2_\text{train}(\bm{P}_{\text{train}}(\bm{\beta},\bm{\gamma}))\) (each of which has two variations of being deterministic or randomised), that worked particularly well with the goal of finding Fixed-angle (CM-)QAOA angles that provide reliable extrapolation to higher lattice dimensions which also provides a significant advantage in solving \svp in the extrapolated dimensions.

\subsubsection{\(c^1_\text{train}\): Maximising the Exponent of the Speedup}
The first approach is to maximise the exponent of the speedup which is equivalent to minimising the exponent of the performance observed on the training set. We thus let
\[
c^1_\text{train}(\bm{P}_{\text{train}}(\bm{\beta},\bm{\gamma})):=a \text{ where } 2^{-am+b} \text{ is the best-fit of }f(m)\text{ to the pairs }\bm{P}_\text{train}(\bm{\beta},\bm{\gamma})
\]
where the best-fit is calculated as explained in \cref{sec:appCalcBestFit_expFit}. This choice of this cost function is better justified because in the extrapolation to higher dimensions we are mostly interested in its asymptotical performance, i.e. the better exponent in the extrapolation, the more suitable is Fixed-angle (CM-)QAOA for solving \svp instances and this is reflected in the cost function used in the training. The disadvantage is that it may happen that an optimiser finds angles \(\bm{\beta},\bm{\gamma}\) so that the results on the training set \(\bm{P}_\text{train}(\bm{\beta},\bm{\gamma})=\left\{P_\text{train}^{m_{\text{start}}}(\bm{\beta},\bm{\gamma}),P_\text{train}^{m_{\text{start}+1}}(\bm{\beta},\bm{\gamma}),\dots,P_\text{train}^{m_{\text{end}}}(\bm{\beta},\bm{\gamma})\right\}\), where \(P_\text{train}^{m_{\text{i}}}(\bm{\beta},\bm{\gamma})\) is a pair
\[P_\text{train}^{m_{\text{i}}}(\bm{\beta},\bm{\gamma})=\left(\begin{array}{c}
	\text{averaged output of Fixed-angle (CM-)QAOAover }\\
	\bm{\mathcal{L}}^{m_i}_{\text{train}}\text{ with angles }\bm{\beta},\bm{\gamma}
\end{array}, m_i\right)\],
do not follow an exponential function while the best-fit of \(a,b\) to the function \(2^{-am+b}\) returns low \(a\). Such angles were observed not to extrapolate well. However, this behaviour has been observed in around a third of the training procedures. They showed a non-efficient performance with too little overlap over the solution, therefore they were discarded. In the remaining ones, the found angles \(\bm{\beta},\bm{\gamma}\) not only found a small \(a\), but also provided results that roughly estimated an exponential function and the extrapolation confirmed the trend.

To avoid over-fitting, we used a modified cost function \(c^\text{1,rand}_\text{train}(\cdot)\) where each iteration of the optimisation has access to only a random subset of both the training dimensions and also to only a random subset of the instances of these dimensions. We experimentally observed that a range about 80\%-90\% for both of the cases performed the best.

\subsubsection{\(c^2_\text{train}\): Maximising the Squared Difference from the Random Guess}

Another choice for  \(c_\text{train}(\cdot)\) that we observed to be working particularly well works by maximising normalised squared distance of the training results \(\bm{P}_\text{train}(\bm{\beta},\bm{\gamma})\) from the function \(2^{-m}\) which represents the time complexity of solving \svp by a naive brute-force enumeration attack.
\begin{align*}
	c^2_\text{train}(\bm{P}_{\text{train}}(\bm{\beta},\bm{\gamma})):=&\sum_{m_\text{start}\leq m\leq m_\text{end}}\big[2^m\big(P_\text{train}^{m_{\text{i}}}(\bm{\beta},\bm{\gamma})_{[1]}-2^{-m}\big)\big]^2\\
	&\ \ \ \ \text{where the \(2^m\) coefficient serves as a normalisation}\\
	&\ \ \ \ \text{to give the difference in each dimension the equal weight}\\
	=&\sum_{m_\text{start}\leq m\leq m_\text{end}}\big[2^mP_\text{train}^{m_{\text{i}}}(\bm{\beta},\bm{\gamma})_{[1]}-1\big]^2
\end{align*}
The notation \(P_\text{train}^{m_{\text{i}}}(\bm{\beta},\bm{\gamma})_{[1]}\) denotes the first element of the pair \(P_\text{train}^{m_{\text{i}}}(\bm{\beta},\bm{\gamma})\) which is the averaged output of Fixed-angle (CM-)QAOA over \(\bm{\mathcal{L}}^{m_i}_{\text{train}}\text{ with angles }\bm{\beta},\bm{\gamma}\).

The performance of \(c^2_\text{train}(\cdot)\) was observed to be comparable to \(c^1_\text{train}(\cdot)\) in terms of the asymptotic speedup observed in the training dataset. Its advantage is that it is less prone to peculiar results that provide an interesting best-fit asymptote but do not follow an exponential function. Its drawback is that it is less justified compared to \(c^1_\text{train}(\cdot)\) because it is only concerned about an improvement (that can be a constant improvement) over time complexity rather than an asymptotical scaling.

Similarly as with \(c^\text{1,rand}_\text{train}(\cdot)\), we have also found it beneficial to avoid over-fitting by using a randomised version \(c^\text{2,rand}_\text{train}(\cdot)\) with the identical randomisation procedure as with \(c^\text{1,rand}_\text{train}(\cdot)\), i.e. each iteration of the optimisation has access to only a random subset of both the training dimensions and also to only a random subset of the instances of these dimensions. Again, we experimentally observed that a range about 80\%-90\% for both of the cases performed the best.

\subsection{Exponential Fitting Approach for the Extrapolation of Fixed-angle (CM-)QAOA performance}\label{sec:appCalcBestFit_expFit}
Given \(\bm{P}(\bm{\beta},\bm{\gamma})=\left\{P^{m_0}(\bm{\beta},\bm{\gamma}),P^{m_1}(\bm{\beta},\bm{\gamma}),\dots,P^{m_{n-1}}(\bm{\beta},\bm{\gamma})\right\}\) where \[P^{m_{\text{i}}}(\bm{\beta},\bm{\gamma})=\left(\begin{array}{c}
	\text{averaged output of Fixed-angle (CM-)QAOAover }\\
	\bm{\mathcal{L}}^{m_i}\text{ with angles }\bm{\beta},\bm{\gamma}
\end{array}, m_i\right)\]
we use analytical approach to find the best-fit of \(P^{m_{\text{i}}}(\bm{\beta},\bm{\gamma})_{[1]}\) to the function \[f(P^{m_{\text{i}}}(\bm{\beta},\bm{\gamma})_{[2]})=2^{-aP^{m_{\text{i}}}(\bm{\beta},\bm{\gamma})_{[2]}+b}\] by determining the constants \(a,b\). The notation \(P^{m_{\text{i}}}(\bm{\beta},\bm{\gamma})_{[k]}\) denotes the \(k\)-th element of the pair \(P^{m_{\text{i}}}(\bm{\beta},\bm{\gamma})\).

We use a widely-used analytical approach to exponential fitting with the least-squares method \cite{leastSquaresFit}. Given a function \(f(m)=2^{-am+b}\) and the pairs \((y_i, m_i)\) to be fitted we proceed to find an analytical solution to constants \(a,b\) that by taking the logarithms on both sides minimise the linearised version of problem:
\begin{align}
	(a,b)&=\argmin_{a,b}\sum_{i=0}^{n-1}\bigl( y_i- f(m_i) \bigr)^2\nonumber\\
	&\approx\argmin_{a,b}\sum_{i=0}^{n-1}\bigl( \log_2 y_i- \log_2 f(m_i) \bigr)^2\nonumber\\
	&=\argmin_{a,b}\sum_{i=0}^{n-1}\bigl( \log_2 y_i+am_i-b \bigr)^2
\end{align}
To find the minimum we calculate the first partial derivatives with respect to \(a\) and \(b\) and set them to \(0\):
\begin{align}
	0&=\frac{\partial}{\partial b}\sum_{i=0}^{n-1}\bigl( \log_2 y_i+am_i-b \bigr)^2=-2\sum_{i=0}^{n-1}\bigl( \log_2 y_i+am_i-b \bigr)\nonumber\\
	&\implies \sum_{i=0}^{n-1} \log_2 y_i+\sum_{i=0}^{n-1}am_i-\sum_{i=0}^{n-1}b =0\nonumber\\
	&\implies nb=\sum_{i=0}^{n-1} \log_2 y_i+\sum_{i=0}^{n-1}am_i\nonumber\\
	&\implies b=\frac{\sum_{i=0}^{n-1} \log_2 y_i+\sum_{i=0}^{n-1}am_i}{n}\label{eq:b_partial}
\end{align}
\begin{align}
	0&=\frac{\partial}{\partial a}\sum_{i=0}^{n-1}\bigl( \log_2 y_i+am_i-b \bigr)^2=2\sum_{i=0}^{n-1}\bigl( \log_2 y_i+am_i-b \bigr)m_i\nonumber\\
	&\implies \sum_{i=0}^{n-1} \log_2 y_i m_i+\sum_{i=0}^{n-1}am_i^2-b\sum_{i=0}^{n-1}m_i =0\nonumber\\
	&\implies \sum_{i=0}^{n-1} \log_2 y_i m_i+\sum_{i=0}^{n-1}am_i^2-\frac{\sum_{i=0}^{n-1} \log_2 y_i+\sum_{i=0}^{n-1}am_i}{n}\sum_{i=0}^{n-1} m_i =0\nonumber\\
	&\implies n\sum_{i=0}^{n-1} \log_2 y_i m_i+na\sum_{i=0}^{n-1}m_i^2-\sum_{i=0}^{n-1} \log_2 y_i\sum_{i=0}^{n-1} m_i-a\left[\sum_{i=0}^{n-1}m_i\right]^2=0\nonumber\\
	&\implies na\sum_{i=0}^{n-1}m_i^2-a\left[\sum_{i=0}^{n-1}m_i\right]^2=\sum_{i=0}^{n-1} \log_2 y_i\sum_{i=0}^{n-1} m_i-n\sum_{i=0}^{n-1} \log_2 y_i m_i\nonumber\\
	&\implies a=\frac{\sum_{i=0}^{n-1} \log_2 y_i\sum_{i=0}^{n-1} m_i-n\sum_{i=0}^{n-1} \log_2 y_i m_i}{n\sum_{i=0}^{n-1}m_i^2-\left[\sum_{i=0}^{n-1}m_i\right]^2}\label{eq:calculated_a}
\end{align}
\begin{align}
	&\ \ \ \text{substituting \Cref{eq:calculated_a} into \Cref{eq:b_partial}}\nonumber\\
	&\implies b=\frac{\sum_{i=0}^{n-1} \log_2 y_i+\frac{\sum_{i=0}^{n-1} \log_2 y_i\sum_{i=0}^{n-1} m_i-n\sum_{i=0}^{n-1} \log_2 y_i m_i}{n\sum_{i=0}^{n-1}m_i^2-\left[\sum_{i=0}^{n-1}m_i\right]^2}\sum_{i=0}^{n-1}m_i}{n}\nonumber\\
	&\implies b=\frac{\sum_{i=0}^{n-1} \log_2 y_i}{n}+\frac{\sum_{i=0}^{n-1} \log_2 y_i\left[\sum_{i=0}^{n-1} m_i\right]^2-n\sum_{i=0}^{n-1} \log_2 y_i m_i\sum_{i=0}^{n-1} m_i}{n^2\sum_{i=0}^{n-1}m_i^2-n\left[\sum_{i=0}^{n-1}m_i\right]^2}\nonumber\\
	&\implies b=\frac{\sum_{i=0}^{n-1} \log_2 y_i\left(n\sum_{i=0}^{n-1}m_i^2-\left[\sum_{i=0}^{n-1}m_i\right]^2\right)+\sum_{i=0}^{n-1} \log_2 y_i\left[\sum_{i=0}^{n-1} m_i\right]^2}{n^2\sum_{i=0}^{n-1}m_i^2-n\left[\sum_{i=0}^{n-1}m_i\right]^2}\nonumber\\
	&\text{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }-\frac{n\sum_{i=0}^{n-1} \log_2 y_i m_i\sum_{i=0}^{n-1} m_i}{n^2\sum_{i=0}^{n-1}m_i^2-n\left[\sum_{i=0}^{n-1}m_i\right]^2}\nonumber\\
	&\implies b=\frac{n\sum_{i=0}^{n-1} \log_2 y_i\sum_{i=0}^{n-1}m_i^2-n\sum_{i=0}^{n-1} \log_2 y_i m_i\sum_{i=0}^{n-1} m_i}{n^2\sum_{i=0}^{n-1}m_i^2-n\left[\sum_{i=0}^{n-1}m_i\right]^2}\nonumber\\
	&\implies b=\frac{\sum_{i=0}^{n-1} \log_2 y_i\sum_{i=0}^{n-1}m_i^2-\sum_{i=0}^{n-1} \log_2 y_i m_i\sum_{i=0}^{n-1} m_i}{n\sum_{i=0}^{n-1}m_i^2-\left[\sum_{i=0}^{n-1}m_i\right]^2}\label{eq:calculated_b}
\end{align}
We have thus found analytic expressions for \(a\) and \(b\) in \Cref{eq:calculated_a} and \Cref{eq:calculated_b} respectively\footnote{Note that this is a widely used approach for an exponential fit. Although the procedure has been widely expanded and accommodated to notation consistent with rest of the work, it cannot be claimed to be our contribution.}. Note that this method does not calculate the optimal \(a\) and \(b\) of least-squares exponential fitting. Because a logarithm was taken to linearise the exponential function, the calculated fit performs a least-squares fit where the errors are scaled logarithmically. This is in our case beneficial as it gives more weight to small errors for large \(m\) than to the large errors of small \(m\), i.e. the fit is more considerate about the fitting the tail of the function.

==> chapters/figures/p_experiment_data/approx_p3_plot_experiments_scaling.tex <==
\begin{axis}[
	ymode=log,
	xmode=linear,
	log basis y={2},
	xmin = 3.8, xmax = 22.2,
	ymin = 7.74624248844371e-08,  ymax = 9,
	xtick distance = 2,
	ytick distance = 4,
	grid = both,
	minor tick num = 1,
	major grid style = {lightgray},
	minor grid style = {lightgray!25},
	width = \textwidth,
	height = \textwidth,
	xlabel = {Lattice basis dimension},
	ylabel = {$\log_{2}$(Overlap with solution)},
	label style={font=\small},
	tick label style={font=\tiny},
	x label style={at={(axis description cs:0.5,0)},anchor=north},
	y label style={at={(axis description cs:0,.5)},anchor=south},
	legend style={at={(0.5,2)},anchor=north,legend cell align=left}]
	
	
	% Plot data from a file
	%\addplot[
	%smooth,
	%thin,
	%red%,
	%dashed
	%] file[skip first] {fc_p_experiment_data/p3_experiments_scaling.dat};
	
	% Plot data from a file
	\addplot [line width=1pt, blue!40]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
	%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	%x index=0,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	%meta index = 9,
	comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p3_experiments_scaling.dat};
	
	
	
	\addplot [line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, blue!40]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	%x index=0,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	%meta index = 9,
	%comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p3_experiments_scaling.dat};
	
	\addplot [line width=1pt, blue!70]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=1,
	header=true,
	comment chars={21}
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_2.dat};
	\addplot [line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, blue!70]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=1,
	header=true,
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_2.dat};
	
	\addplot [line width=1pt, blue!70]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=1,
	header=true,
	comment chars={21}
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_3.dat};
	\addplot [line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, blue!70]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=1,
	header=true,
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_3.dat};
	
		\addplot [line width=1pt, blue!70]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=1,
	header=true,
	comment chars={21}
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_4.dat};
	\addplot [line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, blue!70]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=1,
	header=true,
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_4.dat};
	
	\addplot [line width=1pt, blue!70]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=1,
	header=true,
	comment chars={21}
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_3.dat};
	\addplot [line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, blue!70]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=1,
	header=true,
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_3.dat};
	
	\begin{comment}


	
	\addplot [line width=1pt, blue!100]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=1,
	header=true,
	comment chars={21}
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_7.dat};
	\addplot [line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, blue!100]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		mark size=4pt,
		line width=0.1pt7.dat
	}]
	table[
	smooth,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=1,
	header=true,
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_7.dat};
	
		\end{comment}
	
	
	\addplot[line width=1pt, brown!40]
		plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=4,
	header=true,
	comment chars={21}
	] {chapters/figures/p_experiment_data/p3_experiments_scaling.dat};
			\addplot[line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, brown!40]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=4,
	header=true,
	] {chapters/figures/p_experiment_data/p3_experiments_scaling.dat};

	\addplot[line width=1pt, brown!70]
plot [error bars/.cd, y dir = both, y explicit,
error bar style={line width=0.1pt},
error mark options={
	rotate=90,
	mark size=4pt,
	line width=0.1pt
}]
table[
smooth,
x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
y index=2,
header=true,
comment chars={21}
] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_2.dat};
\addplot[line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, brown!70]
plot [error bars/.cd, y dir = both, y explicit,
error bar style={line width=0.1pt},
error mark options={
	rotate=90,
	mark size=4pt,
	line width=0.1pt
}]
table[
smooth,
x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
y index=2,
header=true,
] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_2.dat};

	\addplot[line width=1pt, brown!70]
plot [error bars/.cd, y dir = both, y explicit,
error bar style={line width=0.1pt},
error mark options={
	rotate=90,
	mark size=4pt,
	line width=0.1pt
}]
table[
smooth,
x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
y index=2,
header=true,
comment chars={21}
] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_3.dat};
\addplot[line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, brown!70]
plot [error bars/.cd, y dir = both, y explicit,
error bar style={line width=0.1pt},
error mark options={
	rotate=90,
	mark size=4pt,
	line width=0.1pt
}]
table[
smooth,
x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
y index=2,
header=true,
] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_3.dat};


	\addplot[line width=1pt, brown!70]
plot [error bars/.cd, y dir = both, y explicit,
error bar style={line width=0.1pt},
error mark options={
	rotate=90,
	mark size=4pt,
	line width=0.1pt
}]
table[
smooth,
x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
y index=2,
header=true,
comment chars={21}
] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_4.dat};
\addplot[line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, brown!70]
plot [error bars/.cd, y dir = both, y explicit,
error bar style={line width=0.1pt},
error mark options={
	rotate=90,
	mark size=4pt,
	line width=0.1pt
}]
table[
smooth,
x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
y index=2,
header=true,
] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_4.dat};
\begin{comment}

	\addplot[line width=1pt, brown!100]
plot [error bars/.cd, y dir = both, y explicit,
error bar style={line width=0.1pt},
error mark options={
	rotate=90,
	mark size=4pt,
	line width=0.1pt
}]
table[
smooth,
x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
y index=2,
header=true,
comment chars={21}
] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_7.dat};
\addplot[line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, brown!100]
plot [error bars/.cd, y dir = both, y explicit,
error bar style={line width=0.1pt},
error mark options={
	rotate=90,
	mark size=4pt,
	line width=0.1pt
}]
table[
smooth,
x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
y index=2,
header=true,
] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_7.dat};
	\end{comment}
	\addplot[line width=0.1pt, red]
table[
smooth,
%thick,
x index=0,
y index=1,
header=false,
] {chapters/figures/line.dat};
	
	\addplot[line width=0.1pt, red]
	table[
	smooth,
	%thick,
	x index=0,
	y index=1,
	header=true,
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_2_line.dat};
	
		\addplot[line width=0.1pt, red]
	table[
	smooth,
	%thick,
	x index=0,
	y index=1,
	header=true,
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_3_line.dat};
	
		\addplot[line width=0.1pt, red]
	table[
	smooth,
	%thick,
	x index=0,
	y index=1,
	header=true,
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_4_line.dat};
	
	\addplot[line width=0.1pt, teal]
	table[
	smooth,
	%thick,
	x index=0,
	y index=2,
	header=false,
	] {chapters/figures/line.dat};
		
	\addplot[line width=0.1pt, teal]
	table[
	smooth,
	%thick,
	x index=0,
	y index=2,
	header=true,
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_2_line.dat};
		
	\addplot[line width=0.1pt, teal]
	table[
	smooth,
	%thick,
	x index=0,
	y index=2,
	header=true,
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_3_line.dat};
	
	\addplot[line width=0.1pt, teal]
	table[
	smooth,
	%thick,
	x index=0,
	y index=2,
	header=true,
	] {chapters/figures/p_experiment_data/approx_p3_experiments_scaling_4_line.dat};
	

\node[blue,] at (175,-20) {\footnotesize$\gamma=1$};
\node[blue,] at (175,-18) {\footnotesize$\gamma=2$};
\node[blue,] at (175,-16) {\footnotesize$\gamma=3$};
\node[blue,] at (175,-5) {\footnotesize$\gamma=4$};

\node[brown,] at (175,-15) {\footnotesize$\gamma=1$};
\node[brown,] at (175,-13.6) {\footnotesize$\gamma=2$};
\node[brown,] at (175,-11.6) {\footnotesize$\gamma=3$};
\node[brown,] at (175,-2.8) {\footnotesize$\gamma=4$};

%\pgfplotstableread[col sep=space]{chapters/figures/p_experiment_data/p3_experiments_scaling.dat}\datatableA
%\pgfplotstableread[col sep=space]{chapters/figures/p_experiment_data/approx_p3_experiments_scaling_2.dat}\datatableB
%\node [brown] at (140,-12.7) {\rotatebox{                 -30.22      }{\small $\alpha=$\pgfplotstablegetelem{1}{alpha_qaoa}\of{\datatableA}\pgfplotsretval}};
%\node [brown] at (140,-10.7) {\rotatebox{                 -30.22      }{\small approx $\alpha=$\pgfplotstablegetelem{1}{alpha_qaoa}\of{\datatableB}\pgfplotsretval}};
%\node [blue] at (140,-18.5) {\rotatebox{                 -30.22      }{\small $\alpha=$\pgfplotstablegetelem{1}{alpha_cm}\of{\datatableA}\pgfplotsretval}};
%\node [blue] at (140,-17.5) {\rotatebox{                 -30.22      }{\small approx $\alpha=$\pgfplotstablegetelem{1}{alpha_cm}\of{\datatableB}\pgfplotsretval}};
	
	\legend{}
\end{axis}

==> chapters/figures/p_experiment_data/p4_plot_experiments_scaling.tex <==
\begin{axis}[
	ymode=log,
	xmode=linear,
	log basis y={2},
	xmin = 3.8, xmax = 22.2,
	ymin = 7.74624248844371e-08,  ymax = 9,
	xtick distance = 2,
	ytick distance = 4,
	grid = both,
	minor tick num = 1,
	major grid style = {lightgray},
	minor grid style = {lightgray!25},
	width = \textwidth,
	height = \textwidth,
	xlabel = {Lattice basis dimension},
	ylabel = {$\log_{2}$(Overlap with solution)},
	label style={font=\small},
	tick label style={font=\tiny},
	x label style={at={(axis description cs:0.5,0)},anchor=north},
	y label style={at={(axis description cs:0,.5)},anchor=south},
	legend style={at={(0.5,2)},anchor=north,legend cell align=left}]
	
	
	% Plot data from a file
	%\addplot[
	%smooth,
	%thin,
	%red%,
	%dashed
	%] file[skip first] {fc_p_experiment_data/p4_experiments_scaling.dat};
	
	% Plot data from a file
	\addplot [line width=1pt, blue]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
	%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	%x index=0,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	%meta index = 9,
	comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p4_experiments_scaling.dat};
	\addplot [line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, blue]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	%x index=0,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	%meta index = 9,
	%comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p4_experiments_scaling.dat};
	
	\addplot[line width=1pt, brown]
		plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p4_experiments_scaling.dat};
	
		\addplot[line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, brown]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
%	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p4_experiments_scaling.dat};
	
			
	\addplot[line width=0.1pt, red]
	table[
	smooth,
	%thick,
	x index=0,
	y index=1,
	header=false,
	] {chapters/figures/line.dat};
	
	\addplot[line width=0.1pt, teal]
	table[
	smooth,
	%thick,
	x index=0,
	y index=2,
	header=false,
	] {chapters/figures/line.dat};
	
		% Plot data from a file
	\addplot [line width=1pt, yellow]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	x index=0,
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p4_opt_experiments_scaling.dat};
	
		\addplot[line width=1pt, orange]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,2
	x index=0,
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p4_opt_experiments_scaling.dat};
	
	\addplot[line width=0.1pt, dashed, blue]
	table[
	%smooth,
	%dashed,
	%thick,
	x index=0,
	y index=7,
	header=true,
	] {chapters/figures/p_experiment_data/p4_experiments_scaling.dat};
	
	\addplot[line width=0.1pt, dashed, brown]
	table[
	%smooth,
	%dashed,
	%thick,
	x index=0,
	y index=8,
	header=true,
	] {chapters/figures/p_experiment_data/p4_experiments_scaling.dat};

\pgfplotstableread[col sep=space]{chapters/figures/p_experiment_data/p4_experiments_scaling.dat}\datatableA
\node [brown] at (140,-15.7) {\rotatebox{                 -30.22      }{\small $\alpha=$\pgfplotstablegetelem{1}{alpha_qaoa}\of{\datatableA}\pgfplotsretval}};
\node [blue] at (140,-18.5) {\rotatebox{                 -30.22      }{\small $\alpha=$\pgfplotstablegetelem{1}{alpha_cm}\of{\datatableA}\pgfplotsretval}};

	
	\legend{}
\end{axis}

==> chapters/figures/p_experiment_data/p5_plot_experiments_scaling.tex <==
\begin{axis}[
	ymode=log,
	xmode=linear,
	log basis y={2},
	xmin = 3.8, xmax = 22.2,
	ymin = 7.74624248844371e-08,  ymax = 9,
	xtick distance = 2,
	ytick distance = 4,
	grid = both,
	minor tick num = 1,
	major grid style = {lightgray},
	minor grid style = {lightgray!25},
	width = \textwidth,
	height = \textwidth,
	xlabel = {Lattice basis dimension},
	ylabel = {$\log_{2}$(Overlap with solution)},
	label style={font=\small},
	tick label style={font=\tiny},
	x label style={at={(axis description cs:0.5,0)},anchor=north},
	y label style={at={(axis description cs:0,.5)},anchor=south},
	legend style={at={(0.5,2)},anchor=north,legend cell align=left}]
	
	
	% Plot data from a file
	%\addplot[
	%smooth,
	%thin,
	%red%,
	%dashed
	%] file[skip first] {fc_p_experiment_data/p5_experiments_scaling.dat};
	
	% Plot data from a file
	\addplot [line width=1pt, blue]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
	%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	%x index=0,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	%meta index = 9,
	comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p5_experiments_scaling.dat};
	\addplot [line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, blue]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	%x index=0,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	%meta index = 9,
	%comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p5_experiments_scaling.dat};
	
	\addplot[line width=1pt, brown]
		plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p5_experiments_scaling.dat};
	
		\addplot[line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, brown]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1ptľ+
	}]
	table[
	smooth,
	%thick,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
%	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p5_experiments_scaling.dat};
	
			
	\addplot[line width=0.1pt, red]
	table[
	smooth,
	%thick,
	x index=0,
	y index=1,
	header=false,
	] {chapters/figures/line.dat};
	
	\addplot[line width=0.1pt, teal]
	table[
	smooth,
	%thick,
	x index=0,
	y index=2,
	header=false,
	] {chapters/figures/line.dat};
	
		% Plot data from a file
	\addplot [line width=1pt, yellow]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	x index=0,
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p5_opt_experiments_scaling.dat};
	
		\addplot[line width=1pt, orange]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,2
	x index=0,
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p5_opt_experiments_scaling.dat};
	
	\addplot[line width=0.1pt, dashed, blue]
	table[
	%smooth,
	%dashed,
	%thick,
	x index=0,
	y index=7,
	header=true,
	] {chapters/figures/p_experiment_data/p5_experiments_scaling.dat};
	
	\addplot[line width=0.1pt, dashed, brown]
	table[
	%smooth,
	%dashed,
	%thick,
	x index=0,
	y index=8,
	header=true,
	] {chapters/figures/p_experiment_data/p5_experiments_scaling.dat};

\pgfplotstableread[col sep=space]{chapters/figures/p_experiment_data/p5_experiments_scaling.dat}\datatableA
\node [brown] at (140,-15.7) {\rotatebox{                 -30.22      }{\small $\alpha=$\pgfplotstablegetelem{1}{alpha_qaoa}\of{\datatableA}\pgfplotsretval}};
\node [blue] at (140,-18.5) {\rotatebox{                 -30.22      }{\small $\alpha=$\pgfplotstablegetelem{1}{alpha_cm}\of{\datatableA}\pgfplotsretval}};

	
	\legend{}
\end{axis}

==> chapters/figures/p_experiment_data/p6_plot_experiments_scaling.tex <==
\begin{axis}[
	ymode=log,
	xmode=linear,
	log basis y={2},
	xmin = 3.8, xmax = 22.2,
	ymin = 7.74624248844371e-08,  ymax = 9,
	xtick distance = 2,
	ytick distance = 4,
	grid = both,
	minor tick num = 1,
	major grid style = {lightgray},
	minor grid style = {lightgray!25},
	width = \textwidth,
	height = \textwidth,
	xlabel = {Lattice basis dimension},
	ylabel = {$\log_{2}$(Overlap with solution)},
	label style={font=\small},
	tick label style={font=\tiny},
	x label style={at={(axis description cs:0.5,0)},anchor=north},
	y label style={at={(axis description cs:0,.5)},anchor=south},
	legend style={at={(0.5,2)},anchor=north,legend cell align=left}]
	
	
	% Plot data from a file
	%\addplot[
	%smooth,
	%thin,
	%red%,
	%dashed
	%] file[skip first] {fc_p_experiment_data/p6_experiments_scaling.dat};
	
	% Plot data from a file
	\addplot [line width=1pt, blue]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
	%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	%x index=0,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	%meta index = 9,
	comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p6_experiments_scaling.dat};
	\addplot [line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, blue]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	%x index=0,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	%meta index = 9,
	%comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p6_experiments_scaling.dat};
	
	\addplot[line width=1pt, brown]
		plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p6_experiments_scaling.dat};
	
		\addplot[line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, brown]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
%	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p6_experiments_scaling.dat};
	
			
	\addplot[line width=0.1pt, red]
	table[
	smooth,
	%thick,
	x index=0,
	y index=1,
	header=false,
	] {chapters/figures/line.dat};
	
	\addplot[line width=0.1pt, teal]
	table[
	smooth,
	%thick,
	x index=0,
	y index=2,
	header=false,
	] {chapters/figures/line.dat};
	
		% Plot data from a file
	\addplot [line width=1pt, yellow]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	x index=0,
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p6_opt_experiments_scaling.dat};
	
		\addplot[line width=1pt, orange]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,2
	x index=0,
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p6_opt_experiments_scaling.dat};
	
	\addplot[line width=0.1pt, dashed, blue]
	table[
	%smooth,
	%dashed,
	%thick,
	x index=0,
	y index=7,
	header=true,
	] {chapters/figures/p_experiment_data/p6_experiments_scaling.dat};
	
	\addplot[line width=0.1pt, dashed, brown]
	table[
	%smooth,
	%dashed,
	%thick,
	x index=0,
	y index=8,
	header=true,
	] {chapters/figures/p_experiment_data/p6_experiments_scaling.dat};

\pgfplotstableread[col sep=space]{chapters/figures/p_experiment_data/p6_experiments_scaling.dat}\datatableA
\node [brown] at (140,-15.7) {\rotatebox{                 -30.22      }{\small $\alpha=$\pgfplotstablegetelem{1}{alpha_qaoa}\of{\datatableA}\pgfplotsretval}};
\node [blue] at (140,-18.5) {\rotatebox{                 -30.22      }{\small $\alpha=$\pgfplotstablegetelem{1}{alpha_cm}\of{\datatableA}\pgfplotsretval}};

	
	\legend{}
\end{axis}

==> chapters/figures/p_experiment_data/p7_plot_experiments_scaling.tex <==
\begin{axis}[
	ymode=log,
	xmode=linear,
	log basis y={2},
	xmin = 3.8, xmax = 20.2,
	ymin = 7.74624248844371e-07,  ymax = 9,
	xtick distance = 2,
	ytick distance = 4,
	grid = both,
	minor tick num = 1,
	major grid style = {lightgray},
	minor grid style = {lightgray!25},
	width = \textwidth,
	height = \textwidth,
	xlabel = {Lattice basis dimension},
	%ylabel = {$\log_{2}$(Overlap with solution)},
	label style={font=\small},
	tick label style={font=\tiny},
	x label style={at={(axis description cs:0.5,0)},anchor=north},
	y label style={at={(axis description cs:0,.5)},anchor=south},
	legend style={at={(0.5,2)},anchor=north,legend cell align=left}]
	
	
	% Plot data from a file
	%\addplot[
	%smooth,
	%thin,
	%red%,
	%dashed
	%] file[skip first] {fc_p_experiment_data/p7_experiments_scaling.dat};
	
	% Plot data from a file
	\addplot [line width=1pt, blue]
%	plot [error bars/.cd, y dir = both, y explicit,
%	error bar style={line width=0.1pt},
%	error mark options={
%		rotate=90,
%		mark size=4pt,
%		line width=0.1pt
%	}]
	table[
	smooth,
	%thick,
	%x index=0,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=1,
	header=true,
	%y error plus index=2,
	%y error minus index=3,
	%meta index = 9,
	comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p7_experiments_scaling.dat};
	\addplot [line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, blue]
	%plot [error bars/.cd, y dir = both, y explicit,
	%error bar style={line width=0.1pt},
	%error mark options={
	%	rotate=90,
		%	red,
	%	mark size=4pt,
	%	line width=0.1pt
	%}]
	table[
	smooth,
	%thick,
	%x index=0,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=1,
	header=true,
	%y error plus index=2,
	%y error minus index=3,
	%meta index = 9,
	%comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p7_experiments_scaling.dat};
	
	\addplot[line width=1pt, brown]
		%plot [error bars/.cd, y dir = both, y explicit,
	%error bar style={line width=0.1pt},
	%error mark options={
	%	rotate=90,
	%	mark size=4pt,
	%	line width=0.1pt
	%}]
	table[
	smooth,
	%thick,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p7_experiments_scaling.dat};
	
		\addplot[line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, brown]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
%	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p7_experiments_scaling.dat};
	
			
	\addplot[line width=0.1pt, red]
	table[
	smooth,
	%thick,
	x index=0,
	y index=1,
	header=false,
	] {chapters/figures/line.dat};
	
	\addplot[line width=0.1pt, teal]
	table[
	smooth,
	%thick,
	x index=0,
	y index=2,
	header=false,
	] {chapters/figures/line.dat};
	

	
	\addplot[line width=0.1pt, dashed, blue]
	table[
	%smooth,
	%dashed,
	%thick,
	x index=0,
	y index=7,
	header=true,
	] {chapters/figures/p_experiment_data/p7_experiments_scaling.dat};
	
	\addplot[line width=0.1pt, dashed, brown]
	table[
	%smooth,
	%dashed,
	%thick,
	x index=0,
	y index=8,
	header=true,
	] {chapters/figures/p_experiment_data/p7_experiments_scaling.dat};

\pgfplotstableread[col sep=space]{chapters/figures/p_experiment_data/p7_experiments_scaling.dat}\datatableA
\node [brown] at (140,-15.7) {\rotatebox{                 -30.22      }{\small $\alpha=$\pgfplotstablegetelem{1}{alpha_qaoa}\of{\datatableA}\pgfplotsretval}};
\node [blue] at (140,-18.5) {\rotatebox{                 -30.22      }{\small $\alpha=$\pgfplotstablegetelem{1}{alpha_cm}\of{\datatableA}\pgfplotsretval}};

	
	\legend{}
\end{axis}

==> chapters/figures/p_experiment_data/p8_plot_experiments_scaling.tex <==
\begin{axis}[
	ymode=log,
	xmode=linear,
	log basis y={2},
	xmin = 3.8, xmax = 22.2,
	ymin = 7.74624248844371e-08,  ymax = 9,
	xtick distance = 2,
	ytick distance = 4,
	grid = both,
	minor tick num = 1,
	major grid style = {lightgray},
	minor grid style = {lightgray!25},
	width = \textwidth,
	height = \textwidth,
	xlabel = {Lattice basis dimension},
	ylabel = {$\log_{2}$(Overlap with solution)},
	label style={font=\small},
	tick label style={font=\tiny},
	x label style={at={(axis description cs:0.5,0)},anchor=north},
	y label style={at={(axis description cs:0,.5)},anchor=south},
	legend style={at={(0.5,2)},anchor=north,legend cell align=left}]
	
	
	% Plot data from a file
	%\addplot[
	%smooth,
	%thin,
	%red%,
	%dashed
	%] file[skip first] {fc_p_experiment_data/p8_experiments_scaling.dat};
	
	% Plot data from a file
	\addplot [line width=1pt, blue]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
	%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	%x index=0,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	%meta index = 9,
	comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p8_experiments_scaling.dat};
	\addplot [line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, blue]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	%x index=0,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	%meta index = 9,
	%comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p8_experiments_scaling.dat};
	
	\addplot[line width=1pt, brown]
		plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	x expr={\thisrow{fixed_used_in_training}==0?nan:\thisrow{x}},
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p8_experiments_scaling.dat};
	
		\addplot[line width=1pt, very thick,dash pattern={on 10pt off 2pt on 5pt off 2pt}, brown]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	x expr={\thisrow{fixed_used_in_training2}==1?nan:\thisrow{x}},
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
%	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p8_experiments_scaling.dat};
	
			
	\addplot[line width=0.1pt, red]
	table[
	smooth,
	%thick,
	x index=0,
	y index=1,
	header=false,
	] {chapters/figures/line.dat};
	
	\addplot[line width=0.1pt, teal]
	table[
	smooth,
	%thick,
	x index=0,
	y index=2,
	header=false,
	] {chapters/figures/line.dat};
	
		% Plot data from a file
	\addplot [line width=1pt, yellow]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,
	x index=0,
	y index=1,
	header=true,
%	y error plus index=2,
%	y error minus index=3,
	comment chars={21}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p8_opt_experiments_scaling.dat};
	
		\addplot[line width=1pt, orange]
	plot [error bars/.cd, y dir = both, y explicit,
	error bar style={line width=0.1pt},
	error mark options={
		rotate=90,
		%	red,
		mark size=4pt,
		line width=0.1pt
	}]
	table[
	smooth,
	%thick,2
	x index=0,
	y index=4,
	header=true,
%	y error plus index=5,
%	y error minus index=6,
	comment chars={21}
	%error expr={symlog(\thisrow{y}+\thisrow{error},\basis)-symlog(\thisrow{y},\basis)}
	%,
	%dashed
	] {chapters/figures/p_experiment_data/p8_opt_experiments_scaling.dat};
	
	\addplot[line width=0.1pt, dashed, blue]
	table[
	%smooth,
	%dashed,
	%thick,
	x index=0,
	y index=7,
	header=true,
	] {chapters/figures/p_experiment_data/p8_experiments_scaling.dat};
	
	\addplot[line width=0.1pt, dashed, brown]
	table[
	%smooth,
	%dashed,
	%thick,
	x index=0,
	y index=8,
	header=true,
	] {chapters/figures/p_experiment_data/p8_experiments_scaling.dat};

\pgfplotstableread[col sep=space]{chapters/figures/p_experiment_data/p8_experiments_scaling.dat}\datatableA
\node [brown] at (140,-15.7) {\rotatebox{                 -30.22      }{\small $\alpha=$\pgfplotstablegetelem{1}{alpha_qaoa}\of{\datatableA}\pgfplotsretval}};
\node [blue] at (140,-18.5) {\rotatebox{                 -30.22      }{\small $\alpha=$\pgfplotstablegetelem{1}{alpha_cm}\of{\datatableA}\pgfplotsretval}};

	
	\legend{}
\end{axis}

==> chapters/figures/table_dataset_dims.tex <==
%p p plot_dim_qs.py
\begin{tabular}{l|rrrrrrrr}
	Lattice Dimension & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9\\
	\hline
	Qubit Count\textsubscript{Non-penalized} & 2 & 6   & 8  & 15 & 18 & 21 & 24 & 36\\
	Qubit Count\textsubscript{Penalized} & 2 & 7  & 10 & 18 & 22 & 26 & 30 & 43\\
\end{tabular}
